Fully Parameterized Quantile Function for Distributional Reinforcement Learning

Distributional Reinforcement Learning (RL) differs from traditional RL in that, rather than the expectation of total returns, it estimates distributions and has achieved state-of-the-art performance on Atari Games. The key challenge in practical distributional RL algorithms lies in how to parameterize estimated distributions so as to better approximate the true continuous distribution. Existing distributional RL algorithms parameterize either the probability side or the return value side of the distribution function, leaving the other side uniformly fixed as in C51, QR-DQN or randomly sampled as in IQN. In this paper, we propose fully parameterized quantile function that parameterizes both the quantile fraction axis (i.e., the x-axis) and the value axis (i.e., y-axis) for distributional RL. Our algorithm contains a fraction proposal network that generates a discrete set of quantile fractions and a quantile value network that gives corresponding quantile values. The two networks are jointly trained to find the best approximation of the true distribution. Experiments on 55 Atari Games show that our algorithm significantly outperforms existing distributional RL algorithms and creates a new record for the Atari Learning Environment for non-distributed agents.

==> rewriting.tex <==
% Three problems to solve:
% 1. all the terminologies. Quantile, Quantile Function, Quantile Regression. Find the best terminology for \tau and \theta.
% 2. How to learn network for \tau and \theta. How is each learning objective derived, to learn the two network. 
% 3. \cite, abbreviation, notation. Try to make the paper more clear, even to someone who don't know RL. 


% First Problem:
% Quantile function: 那个曲线，真值
% Quantile Regression: aims at estimating either the conditional median or other quantiles of the response variable.
% Quantiles: \theta
% Quantiles / return Quantiles
% The \tau th quantile of Y is given by, \tau \in (0, 1)
% Implicit Quantile Network: mapping from probability to quantile, learning the full quantile function, approximating any distribution given sufficient network capacity, a continous map from probabilities to returns.
% Quantization Network: mapping from (state, action) to N probabilities $\tau$, and we learn quantiles for those N probabilities. 
% Given the implicit quantile network, we learn quantization network to select N probabilities $\tau$ in this way, such that the distortion is minimized between the full quantile function(estimated by the implicit quantile network) and the parameterized, quantized distribution.  It is called "Quantile Projection", where we project an arbitrary distribution onto the parameterized space. 
% With the probabilities given by quantization network, we perform quantile regression, to adjust the quantiles at above N probabilities, to minimize the xxx distance to a target distribution. 
% 
% Something is not clear yet ... Let's figure it out. 
% 
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Think a big problem through. Here is the note.
% 
% Quantile regression: Given samples \hat{Z} from distribution for random variable Z, given probability \tau, we want to estimate the \tau 's quantile for random variable Z.  From samples, to quantile estimation.
% Loss for Quantile Regression: Loss_{\tau}(\hat{Z} - \theta), where \hat{Z} is unbiased samples from distribution Z, and \theta is the quantile for accumulative probability \tau. Loss is smoothed, and we can get unbiased estimation of \theta. 
% In RL, \hat{Z} is the target of Bellman update, \theta is the \tau'th quantile for current distribution Z(x,a)
% \hat{Z} must be a unbiased sample from distribution Z. 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Another big problem, the parameterization of QR-DQN, IQN, and OQN. 
%
% QR-DQN, a parameterized quantile distribution, with a set of fixed CDF, and a discrete set of adjustable quantiles, to minimize the xxx distance 
% 
% IQN, learning the quantile function, map from probabilities to quantiles.
% a discrete set of probabilities are sampled, and the corresponding quantiles are adjusted in each update, to adjust the parameter of the IQN. 
% 
% or IQN seems to be a fully parameterization of distribution, but in fact, it is only full quantile function when we have infinity samples. When used, it is combined with a random sampled \tau. And the quantiles at those random sampled \tau is calculated, we approximate target distribution by a parameterized distribution with support at the sampled \tau, and the parameter for IQN is further learned.  
% 
% OQN, what is the parameterization of OQN?
% the full quantile function(Implicit Quantile Network), inherited from IQN 
% Together used with a quantile proposal network, which propose a discrete set of probabilities \tau, the quantiles at those \tau are calculated and updated. We approximate the target distribution with a parameterized distribution with support at the sampled \tau. 
%
%
% 我有一个IQN，它是full quantile function ,但它并不是真的那个用于更新的参数化的概率分布。只有当quantile数目趋于无穷，它才是一个逼近真实分布的曲线。
% 实际使用的时候，我从(0,1) sample一些probabilities， 我从IQN把对应的quantile取出来，我还是用一组diracs的分布去逼近一个target分布，我对quantile的更新会传导到IQN本身的mapping参数上去。
% 
% 既然都是有限的集合，都是用一组diracs的分布去逼近一个target分布，sampled \tau没有理由比fixed \tau就一定好了，而理论上最好的那个\tau，当然是在有限support情况下，最完美逼近target分布的那个\tau. 
%
% Target分布我们不知道，我们用当前(s,a)的IQN的那个分布替代好了，近似一下
% 最优的\tau要求积分，没法求，我们推导了一个等式出来，满足这个等式并且满足二阶hessian条件，我们就能得到optimal \tau. 
% 实用中，我们就最小化这个条件的loss，来学习一组尽可能满足这个条件的\tau， 优化目标的学习信号，传导到了\tau的那个network上，我们就学习了quantiles proposal network.
%
% 一个问题，如果你的IQN都只在optimal \tau上学习过，见过样本，没有利用相信IQN的那根曲线，可以很好的拟合曲线，很好的用来推导出来最优的\tau. 
% 回答：随着stochastic优化，Quantile proposal network总会输出一样不一样的\tau, 所以IQN是有机会见到各种\tau的，也有机会学到各种\tau下曲线的形状，因而也会有部分能力推导出来最优的\tau. 
% 反正近似挺多的，用实验结果说话吧！

% Another big problem solved, now we understand what is the parameterization 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A modification to IQN, 
% We propose to optimize the CDF \tau to best approximate the full quantile function with limited number of quantiles, rather than fixed, uniform \tau in QR-DQN or random sampled \tau in IQN. 
% 1. good for Q expectation, 2. good for update full quantile function. 
% By optimizing \tau, we can approximate the full quantile function under limited number of quantiles. We can derive the sample mean which is closer to the expectation under the same number of samples, which is useful when we estimate the expected Q from the full quantile function. We also identify the best locations of cdfs to adjust quantiles during learning. The optimized \tau are assumed to best represent the whole quantile function, and update the quantile function at those \tau are assumed to be more efficient than update a random \tau.  


%Towards this end, we propose to learn a quantile proposal network $T(s,a)$, to propose best \taus for each state-action pair. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract: 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rather than fixed or sampled probabilities, select the discrete set of probabilities with the aim at minimizing the xxx distance between target distribution and parameterized distributions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Introduction: 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% rather than fixed or sampled probabilities, optimizing the discrete set of probabilities with the aim at minimizing the xxx distance between target distribution and parameterized distributions.
% quantile target proposal network(QTPN): generate a discrete set of probabilities.
% implicit quantile network(IQN): learn the mapping from quantiles to probabilites.
% 1. learn QTPN, minimizing the xxx distance between target distribution and parameterized distribution. 
% problem 1.1, xxx distance can not be optimized by stochastic gradient descent, there is an intergration.
%            we solve this problem by deriving the optimal condition for probabilities that optimize the distribution, and we optimize \tau by minimize the error of the condition.
% problem 1.2, in RL the full quantile function of target distribution is not avaible. 
%            we use the IQN of current state-action pair, as an estimation of the target distribution, and use it approximately.
% In total, two approximation is made here. 
% 2. learn IQN,  quantile regression on learned target probabilities.
% we are actually adjusting the IQN on the specific target probabilities generated by QTPN. Intuitively speaking, we believe those points can represent the distribution best and is the best set of data points to train. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Background
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 1. MDP
% 2. Z, bellman update, with the whole distribution
% 3. XXX distance. convergence result, contraction in xxx distance. 
% 4. Parameterization: Quantile Regression(let's skip C51 here.)
%    fixed support in QR-DQN
%    random support in IQN
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Method
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parameterization: learn to optimize that support on both side, probability and quantile. QTPN, generate probability for each state-action pair; IQN, generate quantile for each state-action pair and given probability. Together, generate a parameterized distribution with N support, for each-state action pair. 
% (这里的重点，在于越过IQN似乎能够刻画整个quantile function的表面，意识到它事实上也是一个QR的setting，用了一组离散的probabilities，来参数化分布，并且进行运算. IQN只是在运算的结果上，进一布在有限数据点算了从probabilities到 quantile的mapping，仅此而已。
%基于离散点的参数化的分布，一个network算一个参数，一个network算另一个参数，也十分的自然了。)
% How to learn QTPN: learn to optimized the proposed probabilities, \tau. Quantile projection, project a target distribution to a parameterized distribution space, by minimizing the xxx distance. Two approximations are made here: 1. target distribution unknown, we use current distribution as approximation. 2. objective function cannot be optimized, we derive the optimal condition and optimize the condition to be hold. x-axis 
% How to learn IQN: learn to optimized the quantiles, \theta, quantile regression, estimating quantiles given samples from target distribution, TD error and huber loss from quantile regression. y-axis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% What did we do?
% select support points on probability side for parameterized distribution, by minimizing the distortion(1-Wasserstein distance) between target distribution and parameterized distribution, with target distribution unknown therefore approximated by current distribution, with the objective function intractable therefore we optimize the optimal condition. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% to-do list 1 : get all the terminologies done. Quantile, Quantile Function, Quantile Regression. Find the best terminology for \tau and \theta.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%We “transpose” the parametrization from C51: whereas the former uses N fixed locations for its approximation distribution and adjusts their probabilities, we assign fixed, uniform probabilities to N adjustable locations;

%The C51 algorithm models Zπ(x, a) using a discrete distribution supported on a “comb” of fixed locations z1 ≤· · · ≤ zN uniformly spaced over a predetermined interval.The parameters of that distribution are the probabilities qi, expressed as logits, associated with each location zi

%Recall that C51 approximates the distribution at each state by attaching variable (parametrized) probabilities q1, . . . , qN to fixed locations z1 ≤ · · · ≤ zN .

%Our approach is to “transpose” this parameterization by considering fixed probabilities but variable locations. Specifically, we take uniform weights, so that qi = 1/N for each i = 1, . . . , N

%Effectively, our new approximation aims to estimate quantiles of the target distribution. Accordingly, we will call it a quantile distribution, and let ZQ be the space of quantile distributions for fixed N. We will denote the cumulative probabilities associated with such a distribution (that is, the discrete values taken on by the CDF) by τ1, . . . , τN , so that τi = i N for i = 1, . . . , N. We will also write τ0 = 0 to simplify notation

%A quantile distribution Zθ ∈ ZQ maps each state-action pair (x, a) to a uniform probability distribution supported on {θi(x, a)}.

%Compared to the original parametrization, the benefits of a parameterized quantile distribution are threefold. we are not restricted to prespecified bounds on the support, or a uniform resolution

%In our case, we analyze the distributional Bellman update, projected onto a parameterized quantile distribution,

%Let Y be a distribution with bounded first moment and U a uniform distribution over N Diracs as in (7), with support {θ1, . . . , θN }. 

%, for quantile τ //but, quantile actually refers to \theta, instead of \tau.

% the quantile function F−1Z(τ )

% quantile function, a continuous map from probabilities to returns.

% These algorithms are restricted to assigning probabilities to an a priori fixed, discrete set of possible returns. Dabney et al. (2018) propose an alternate pair of choices, parameterizing the distribution by a uniform mixture of Diracs whose locations are adjusted using quantile regression. Their algorithm, QR-DQN, while restricted to a discrete set of quantiles, automatically adapts return quantiles to minimize the Wasserstein distance between the Bellman updated and current return distributions. This flexibility allows QR-DQN to significantly improve on C51’s Atari-57 performance.

%Bellemare et al. (2017) parameterize the return distribution as a categorical distribution over a fixed set of equidistant points and minimize the KL divergence to the projected distributional Bellman target.

%The categorical parameterization

%quantile targets, \hat{\tau}, the only good terminology for \tau.

%quantile estimates, \theta

% respective quantile values

% In mathematics, the support of a real-valued function f is the subset of the domain containing those elements which are not mapped to zero. If the domain of f is a topological space, the support of f is instead defined as the smallest closed set containing all points not mapped to zero. This concept is used very widely in mathematical analysis. 不能乱用， 特指非零的部分

% Summary:
% \tau: quantile targets, (\tau_i + \tau_{i+1})/2;  fixed, uniform probabilities;  cumulative probabilities associated with such a distribution;  
% \theta: return quantile, respective quantile value, quantile estimates, quantiles, 
% C51: assigning probabilities to an a priori fixed, discrete set of possible returns; parameterize the return distribution as a categorical distribution over a fixed set of equidistant points
% QR-DQN: parameterizing the distribution by a uniform mixture of Diracs whose locations are adjusted using quantile regression

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% to-do list 2 : get all equations and notations done. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


